Radio Pulsar Emission-Beam Geometry at Low Frequency: LOFAR High Band Survey Sources Studied using Arecibo at 1.4 GHz and 327 MHz

This paper continues our study of radio pulsar emission-beam configurations with the primary intent of extending study to the lowest possible frequencies. Here we focus on a group of 133 more recently discovered pulsars, most of which were included in the (100-200 MHz) LOFAR High Band Survey, observed with Arecibo at 1.4 GHz and 327 MHz, and some observed at decameter wavelengths. Our analysis framework is the core/double-cone beam model, and we took opportunity to apply it as widely as possible, both conceptually and quantitatively, while highlighting situations where modeling is difficult, or where its premises may be violated. In the great majority of pulsars, beam forms consistent with the core/double-cone model were identified. Moreover, we found that each pulsar's beam structure remained largely constant over the frequency range available; where profile variations were observed, they were attributable to different component spectra and in some instances to varying conal beam sizes. As an Arecibo population, many or most of the objects tend to fall in the Galactic anticenter region and/or at high Galactic latitudes, so overall it includes a number of nearer, older pulsars. We found a number of interesting or unusual characteristics in some of the pulsars that would benefit from additional study. The scattering levels encountered for this group are low to moderate, apart from a few pulsars lying in directions more toward the inner Galaxy.

==> junk.tex <==
\begin{figure*}
\begin{flushleft}
{\bf 1. CORRECTED GROUP B PROFILES}
\vspace{12 pt}
\end{flushleft}
\begin{center}
\begin{tabular}{@{}ll@{}ll@{}}
{\mbox{\includegraphics[width=52mm,height=53mm]{plots/J0611+30_Bmodel.ps}}}&
{\mbox{\includegraphics[width=50mm,height=53mm]{plots/J1819+1305_Bmodel.ps}}}& \ \ \ 
\\
{\mbox{\includegraphics[width=52mm]{plots/J0611+30P.ps}}}&
{\mbox{\includegraphics[width=52mm]{plots/J1819+1305P.ps}}}& \ \ \ 
{\mbox{\includegraphics[width=52mm]{plots/J1915+0738P.ps}}}\\
{\mbox{\includegraphics[width=52mm]{plots/J0611+30L.ps}}}& 
{\mbox{\includegraphics[width=52mm]{plots/J1819+1305L.ps}}}& \ \ \
{\mbox{\includegraphics[width=52mm]{plots/J1915+0738L.ps}}}\\
\end{tabular}
\caption{Beam size models and average profiles for  PSRs J0611+30 (1420-MHz CORRECTED), J1819+1305 and J1915+0738 (both 327-MHz CORRECTED).
Plotted values represent the \textit{scaled} inner (blue) and outer (cyan) conal beam radii and the core angular diameter (red), respectively, and are logarithmic on both axes (see text). The nominal values of the three beam dimensions at 1 GHz are shown in each plot by a small triangle. The yellow hatching indicates an average scattering level (with an orange 10X line), and the orange hatching indicates measured scattering times (both where applicable). The top panel in each of the average profiles (second two rows) is the average profile, with the solid line (black) showing the total intensity, the dashed line (green) showing the linear polarization, and dotted (red) line showing the circular polarization. The bottom panels show the polarization angle against longitude.}
\label{figA1}
\end{center}
\end{figure*}

\begin{figure*}
\begin{center}
\begin{tabular}{@{}ll@{}ll@{}}
{\mbox{\includegraphics[width=52mm]{plots/J1919+0134_Bmodel.ps}}} &{\mbox{\includegraphics[width=52mm]{plots/J1953+1149_Bmodel.ps}}}& \ \ \
{\mbox{\includegraphics[width=52mm]{plots/J2007+0910_Bmodel.ps}}} \\
{\mbox{\includegraphics[width=52mm]{plots/J1919+0134P.ps}}} &
{\mbox{\includegraphics[width=52mm]
{plots/J1953+1149P.ps}}}& \ \ \  
{\mbox{\includegraphics[width=52mm]{plots/J2007+0910P.ps}}} \\ 
{\mbox{\includegraphics[width=52mm]{plots/J1919+0134L.ps}}} &{\mbox{\includegraphics[width=52mm]{plots/J1953+1149L.ps}}}& \ \ \ 
{\mbox{\includegraphics[width=52mm]{plots/J2007+0910L.ps}}} \\ 
\end{tabular}
\caption{Scaled beam dimensions and average profiles for PSRs J1919+0134, J1953+1149 and J2007+0910 (all 327-MHz CORRECTED) as in Fig.~\ref{figA1}.}
\label{figA2}
\end{center}
\end{figure*}

\begin{figure*}
\begin{center}
\begin{tabular}{@{}ll@{}ll@{}}
{\mbox{\includegraphics[width=52mm]{plots/J2008+2513_Bmodel.ps}}} &{\mbox{\includegraphics[width=52mm]{plots/J2045+0912_Bmodel.ps}}}& \ \ \
{\mbox{\includegraphics[width=52mm]{plots/J2156+2618_Bmodel.ps}}} \\
{\mbox{\includegraphics[width=52mm]{plots/J2008+2513P.ps}}} &{\mbox{\includegraphics[width=52mm]{plots/J2045+0912P.ps}}}& \ \ \  
{\mbox{\includegraphics[width=52mm]{plots/PQpJ2156+2618.53377pa0.ps}}} \\ 
{\mbox{\includegraphics[width=52mm]{plots/J2008+2513L.ps}}} &
{\mbox{\includegraphics[width=52mm]{plots/J2045+0912L.ps}}}& \ \ \
{\mbox{\includegraphics[width=52mm]{plots/J2156+2618L.ps}}} \\ 
\end{tabular}
\caption{Scaled beam dimensions and average profiles for PSRs J2008+2513, J2045+0912 and J2156+2618 (all 327-MHz CORRECTED) as in Fig.~\ref{figA1}.}
\label{figA3}
\end{center}
\end{figure*}

\begin{figure*}
\begin{center}
\begin{tabular}{@{}ll@{}ll@{}}
{\mbox{\includegraphics[width=52mm]{plots/J2243+1518_Bmodel.ps}}} \\
{\mbox{\includegraphics[width=52mm]{plots/J2234+2114P.ps}}}& \ \ \ {\mbox{\includegraphics[width=52mm]{plots/J2248-0101P.ps}}}\\ 
{\mbox{\includegraphics[width=52mm]{plots/J2243+1518L.ps}}} & \ \ \ {\mbox{\includegraphics[width=52mm]{plots/J2248-0101L.ps}}}\\ 
\end{tabular}
\caption{Scaled beam dimensions and average profiles for J2243+1518 (1400-MHz CORRECTED) and PSRs J2248--0101 (324-MHz CORRECTED), as in Fig.~\ref{figA1}.}
\label{figA4}
\end{center}
\end{figure*}

\label{lastpage}
